Localization and Mapping using Instance-specific Mesh Models

This paper focuses on building semantic maps, containing object poses and shapes, using a monocular camera. This is an important problem because robots need rich understanding of geometry and context if they are to shape the future of transportation, construction, and agriculture. Our contribution is an instance-specific mesh model of object shape that can be optimized online based on semantic information extracted from camera images. Multi-view constraints on the object shape are obtained by detecting objects and extracting category-specific keypoints and segmentation masks. We show that the errors between projections of the mesh model and the observed keypoints and masks can be differentiated in order to obtain accurate instance-specific object shapes. We evaluate the performance of the proposed approach in simulation and on the KITTI dataset by building maps of car poses and shapes.

==> tex/Approach_Perception.tex <==


\subsection{Semantic Perception}
\label{sec:approach_perception}


Class-level and instance-level features are detected from camera images. For each frame, we first use \cite{chen2018encoder} to get a segmentation mask where each pixel is assigned to zero as background or one of the class labels in $\mathcal{C}=\{1...C\}$. Then instance-specific information is collected from object and keypoint detectors in \cite{chen2018deeplab} and \cite{pavlakos20176}. The $k$-th detected result in this frame can be represented as 
\begin{align*}\mathcal{S}_k=(S_{k}^c, S_{k}^{bbx}, S_{k}^u, S_{k}^{kp}, S_{k}^{q})\end{align*}
Here $S_{k}^c\in\mathcal{C}$ stands for the instance class, $S_{k}^{bbx} \in\mathbb{R}^4$ defines 2D location, width and height of the bounding box, $S_{k}^u\in{[0,1]}$ measures the object detection uncertainty and finally $S_{k}^{kp} \in \mathbb{R}^{N \times 2}$ and $S_{k}^{q} \in \mathbb{R}^{N\times 1}$ represent keypoints' 2D locations and detection qualities respectively, where $N$ is the total number of keypoints for the corresponding class $S_k^c$ (here we use $N$ to denote $N^{S_k^c}$ for brevity). 

Data association for instances is needed for both temporal tracking and spatial matching when stereo camera is used. We implemented a method based on the image processing frontend in \cite{sun2018robust}. Same algorithm can be extended to other camera settings (RGBD or monocular cameras) with slight modifications. The methodology here is to associate keypoints in the tracked instance to the most probable bounding box from current observations. Take spatial tracking for the $i$-th instance in the left camera ${}^L\mathcal{S}_i$ as an example, we first use KLT optical flow algorithm \cite{lucas1981iterative} for stereo matching to estimate keypoints' locations in the right camera $\overline{{}^RS^{kp}_i} \in \mathbb{R}^{N\times 2}$ with a stereo inlier mask $\mathcal{B}_i \in \mathbb{B}^{1\times N}$ where $\mathbb{B}$ stands for Boolean domain defined as 0 for outliers and 1 for inliers. Then for the $j$-th observation from the right camera, we create another mask $B^b_{i,j}\in \mathbb{B}^{1\times N}$ to tell whether each keypoint in $\overline{{}^R S^{kp}_i}$ is within the bounding box of that observation. Eventually we calculate the matching score as
\begin{align*}
M_{i,j}=B^s_i\odot B^b_{i,j} \cdot {}^LS^q_i
\end{align*}
We select the observation in right camera with bounding box owning the highest matching score. If that observation shares the same class with the tracked instance and the observed bounding box is in proper width and height, we say that instance has been successfully matched. Otherwise we declare that instance loses tracked. As for spatial tracking, we also use the KLT algorithm to estimate keypoints' location of previous tracked instance in current frame, with a mask indicating inliers, and perform the same procedures mentioned above.

% \YUE{is it okay to add that many symbols here?}

==> tex/Review_Semantic.tex <==
\subsection{Semantic Information}


Detecting semantic representation from image data has been a hot topic in computer vision and robotics. The ultimate goal is to tell what and where the objects are in the scene.  Semantic concepts can be seen as a high-level understanding to the environment which preserves potential advantages in complex tasks like navigation or human-robot interaction \cite{cadena2016past}. Semantic information can be obtained from object detection, semantic segmentation and keypoint detection. In temporal observations like videos, we also need tracking method to find data association between frames.

Object detection is to classify and localize multiple objects in a single image. Detection results are presented in class labels and upright bounding boxes. Traditional methods utilize hand-craft features and stage-by-stage shallow architecture in learning procedures \cite{felzenszwalb2010object}, whereas state-of-art approaches use deep neural networks in an end-to-end process to achieve better performance \cite{ren2015faster, redmon2018yolov3, liu2016ssd, he2017mask, cai2017cascade}. However, bounding boxes only provide a coarse estimation for the objects’ position and scale, which can be heavily biased when detecting irregular shapes or not upright aligned objects (e.g. a broom in the corner).

Semantic segmentation is a dense method to perceive object classes from the scene\cite{garcia2017review}. It assigns each pixel in the image to a class label, hence renders semantic masks with respect to each class. \cite{Long_2015_CVPR} first designed a convolutional networks with deconvolution layers and skip connections for semantic segmentation. \cite{badrinarayanan2015segnet} introduced a general encoder-decoder structure for better performance. \cite{yu2015multi} used dilated convolution to replace pooling layers for multi scale aggregation. \cite{chen2018deeplab} added fully connected conditional random field for structured prediction and adopt atrous spatial pyramid pooling to handle multi-scale objects. \cite{chen2018encoder} linked advanced spatial pyramid pooling module \cite{chen2017rethinking} to a decoder structure \cite{badrinarayanan2015segnet} with Xception \cite{chollet2017xception} as backbone to achieve leading performance.

Recent datasets \cite{xiang_wacv14, lin2014microsoft, andriluka20142d} and deep learning model \cite{newell2016stacked} make it possible to extract semantic point features inside bounding boxes or from images with a single object. Each semantic keypoint represents a specific corresponding part (e.g. left front wheel or right back tail light) from an object (e.g. car). Compared to basic geometric features \cite{lowe1999object, dalal-triggs, rublee2011orb}, semantic keypoints own uniqueness in both class-level and in component-level, therefore bring in potential value in downstream tasks. \cite{newell2016stacked} used semantic keypoints for human pose estimation. \cite{pavlakos20176} leveraged category-specific keypoints and 3D CAD models for six degree of freedom pose estimation.
